Retargeting Visual Data with Deformation Fields

Seam carving is an image editing method that enable content-aware resizing, including operations like removing objects. However, the seam-finding strategy based on dynamic programming or graph-cut limits its applications to broader visual data formats and degrees of freedom for editing. Our observation is that describing the editing and retargeting of images more generally by a displacement field yields a generalisation of content-aware deformations. We propose to learn a deformation with a neural network that keeps the output plausible while trying to deform it only in places with low information content. This technique applies to different kinds of visual data, including images, 3D scenes given as neural radiance fields, or even polygon meshes. Experiments conducted on different visual data show that our method achieves better content-aware retargeting compared to previous methods.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/feedback_needed.tex <==
\section{State and Todo}
\subsection{Final steps:}
	DELTE SUPLEMENTAL PAGES FROM SUBMISSION\\
    Sync abstract here and in website\\
    Shorten to 8 pages\\
	Finish writing appendix \todo{20 m}\\
    SUPPLEMENTAL
 
\subsection{Planned Supplemental}
Code Example\\~\\
Video explanation\\~\\
Animation of training in 2D and 3D\\
Gradually applinyg 2D/3D deformation\\
Deforming a 3D scene in two different directions\\
Animations in more pretty (don't fly straight)

==> sec/fig_table/fig_2d_comp.tex <==
\begin{figure}[t!]
    \centering
    {
       % \begin{adjustbox}{width=\linewidth,center}
            \setlength\tabcolsep{0pt}
        \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}} cccc }
                
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}
                \\
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}
                \\
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}
                \\
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}&
                \includegraphics[width=0.19\linewidth]{example-image}
                \\
                {(a)~Input}{}&
                {(b)~Cropped}{}&
                {(c)~Seam Carving}{}&
                {(d)~Ours}{}\\
            \end{tabular*}
       % \end{adjustbox}
    }
    \caption{
        Qualitative comparison of seam carved results on 2D images by different methods. 
    }
    \label{fig:2d_comp}
\end{figure}

==> sec/figures/deformation_field.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{images/dummy.png}
\caption{Example of how our deformation fields work.}\label{fig:deformation_field_problem}
\end{figure}

==> sec/figures/energy.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{images/ptc_energy.png}
\caption{View and depth map (left), resulting point cloud with energy values (brighter red means more energy, centre), and smoothed point cloud with energy values (right).}\label{fig:energy_ptc_and_smoothed_ptc}
\end{figure}

==> sec/figures/inversion.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{images/dux.png}
\caption{Learned offset $D(x)$ that maps a point $x$ to $x'$, with $U(x')$ giving the inverse of the offset. Note that as we only sample sparsely and our deformation map is a monotonic function, a point position is only relevant after being deformed and hence, we need to not sample points on the surface, but points that are being deformed to be on the surface \textbf{after} deformation.}\label{fig:inversion}
\end{figure}

==> sec/figures/nerf_scenes.tex <==
\begin{figure}[h]
\centering
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/ex_farm.png}\\
        \includegraphics[width=\textwidth]{images/harbour_seamed.png}\\
    \end{subfigure}
\caption{Applying our retargeting to NeRFs. Top row: Input, stretched, retargeted with our method. Bottom row: Input, folds on the input suggested by our approach, retargeted with our method.}\label{fig:seam_nerfs}
\end{figure}

==> sec/figures/pipeline_images.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=1.0\textwidth]{images/svg/pipeline_general.pdf}
\caption{Our proposed Pipeline for images: We train a neural field to represent the image, and a neural field to represent the cumulative gradient. We then optimise the deformation to not skip over content with high rate of colour change (\ie semantically meaningful).}\label{fig:pipeline_images}
\end{figure*}
